Transformer-Based Temporal Information Extraction and Application: A Review

Temporal information extraction (IE) aims to extract structured temporal information from unstructured text, thereby uncovering the implicit timelines within. This technique is applied across domains such as healthcare, newswire, and intelligence analysis, aiding models in these areas to perform temporal reasoning and enabling human users to grasp the temporal structure of text. Transformer-based pre-trained language models have produced revolutionary advancements in natural language processing, demonstrating exceptional performance across a multitude of tasks. Despite the achievements garnered by Transformer-based approaches in temporal IE, there is a lack of comprehensive reviews on these endeavors. In this paper, we aim to bridge this gap by systematically summarizing and analyzing the body of work on temporal IE using Transformers while highlighting potential future research directions.

==> Tables/time-expression-methods.tex <==
\begin{table*}
\small
\centering
\begin{tabular}{l l l p{3cm} p{4cm} c}
\toprule
\textbf{Work} & \textbf{Base Model} & \textbf{Task} & \textbf{Approach} & \textbf{Eval.} & \textbf{Model Avail.}\\
\midrule
\citet{chen2019exploring} & BERT & Ident. & Token Class. & Newswire Text, Wikipedia Articles & \XSolidBrush \\
\citet{kim-etal-2020-time} & BERT & Norm. & Seq. Class. & Fictional books & \XSolidBrush \\
\citet{laparra-etal-2021-semeval} & RoBERTa & Ident. & Token Class. & Food Security Text & \Checkmark \\
\citet{mirzababaei-etal-2022-hengam} & RoBERTa & Ident. & Token Class. & Persian NER Datasets & \XSolidBrush \\
\citet{olex2022temporal} & BERT & Ident. & Token Class. & Clinical Text &  \Checkmark \\
\citet{almasian2022time} & ELECTRA & Ident. & Token Class. & Newswire Text & \XSolidBrush \\
\citet{cao-etal-2022-xltime} & mBERT, XLMR & Ident. & Token Class. & Newswire Text, Wikipedia Articles, Twitter Text & \Checkmark \\
\citet{shwartz-2022-good} & BERT & Norm. & MLM & Twitter Text & \XSolidBrush \\
\citet{lange-etal-2023-multilingual} & XLM-R & Ident., Norm. & Token Class. (Ident.), MLM (Norm.) & Newswire text, Wikipedia Articles & \Checkmark \\
\bottomrule
\end{tabular}
\caption{Overview of time expression identification and normalization methods.}
\label{table:time-expression-methods}
\end{table*}


==> sections_old/abstract.tex <==
\begin{abstract}
This document is a supplement to the general instructions for *ACL authors. It contains instructions for using the \LaTeX{} style files for ACL conferences. 
The document itself conforms to its own specifications and is, therefore, an example of what your manuscript should look like.
These instructions should be used both for papers submitted for review and for final versions of accepted papers.
\end{abstract}

==> sections_old/applications.tex <==
\section{Downstream-Task Applications}

==> sections_old/experiments.tex <==
\section{Experiments}

\subsection{Research Questions}

\begin{enumerate}
    \item Has the recently emerged closed-source large language model solved temporal relation extraction?
    \item If we want to use an open-source large language model to solve the task of temporal relation extraction, which model should we start with, and which dataset should we use? %, not a science question
    \item What are the main errors made by these open-source large language models (do we still need constraints)?
    \item Have they solved in the fine-tuning setting?
    \item Have they solved in the few-shot setting?
    \item Which of the prior works still provide benefits in LLM (adv loss, pick the easiest method to implement)?
\end{enumerate}

==> sections_old/introduction.tex <==
\section{Introduction}
Temporal reasoning involves the ability to extract and comprehend time-related information, construct events in a logical time order, and integrate the temporal aspect into intricate tasks like question answering and causal inferences. This ability is particularly critical in the clinical field for patient diagnosis and treatments (references), as well as finance for making time-sensitive decisions (references).
 
Temporal reasoning as an important NLP domain has been covered in several survey papers. Sanampudi and Kumari (2010), Leeuwenberg and Moens (2020), Olex and McInnes (2021), and Alfattni, Peek, and Nenadic (2020) have explored various aspects of temporal representation, including basic temporal relations like qualitative Interval Algebra and the INDU framework, diverse annotation schemas such as TIMEX2, Chronos, and TimeML, and models for the event relation prediction task, ranging from traditional machine learning models like Markov logic network, SVM, and CRF to recent neural networks like LSTM and transformers. In addition to event relation prediction, Olex and McInnes (2021) also introduced other temporal-related tasks like temporal expression recognition, event recognition tasks, timeline visualization, and the model architectures applied in this field. 

The existing surveys primarily focus on the limited scope of temporal reasoning -- information extraction tasks (event/time expression identification, event relation classification). In addition, there is a lack of specificity and depth in the analysis and comparison of contributions from different systems and approaches resulting in insufficient guidance on future research directions. 

The aim of this survey is to address the existing gap in the field by accomplishing the following:
\begin{itemize}
    \item Expanding the scope of temporal reasoning tasks that are examined in the survey, including tasks related to information extraction, complex temporal question answering, common knowledge reasoning, and next event prediction.
    \item Comparing recent systems by highlighting the key trends, contributions, and potential drawbacks.
    \item Presenting the performance of T5-3B and GPT4 as straightforward yet robust baseline models for each task.
    \item Identifying future directions for further improvement in view of the baseline models.  
\end{itemize}



==> sections_old/related-works.tex <==
\section{Related Works}
...


==> sections_old/temporal-relation-extraction.tex <==
\section{Temporal Relation Extraction}
The goal of the temporal relation extraction is to construct a directed acyclic graph given a text document.
The nodes are temporal entities, which can be an event or a time
The edges are temporal relations.
Most of the temporal relations used in existing works are derived from the 13 relations in Allen's interval algebra.
Temporal relations can be grouped according to the types of temporal entities involved: 1) event-event relations, 2) event-time relations, and 3) time-time relations.
The relations in the temporal graph need to follow two temporal-specific rules:
\begin{enumerate}
    \item Symmetry: Some temporal relationships exhibit symmetry, such as before, after, and equal. For example, if A is before B, then B is after A. If A is equal to B, then B is also equal to A.
    \item Transitivity: If A is before B, and B is before C, then A is before C.
\end{enumerate}

The typical temporal relation extraction method treats this task as a pairwise classification problem. Given two temporal entities, a classifier learns to identify the temporal relationship between them (Section x.x). Based on the pairwise classifier, existing works have proposed various methods to impose temporal rules during training and testing, aiming to improve the global consistency of the model's predictions (Section x.x). Additionally, there are a few studies that present alternative frameworks for the temporal relation extraction task, which are discussed in Section x.x.

\subsection{Pairwise Classification Approaches}
\subsubsection{Feature-based Machine Learning Approaches}

% add examples for the features, cite one paper and explain it
% should have an example for explanation.

The early pairwise temporal classification works \cite{bramsen-etal-2006-inducing, bethard-etal-2007-timelines, chambers-jurafsky-2008-jointly, do-etal-2012-joint, bethard-2013-cleartk, laokulrat-etal-2013-uttime, chambers-etal-2014-dense} primarily employ machine learning models trained on human-annotated or externally extracted features of temporal entities and their context. These features typically include lexical, syntactic, and semantic features, as well as input temporal entities' attributes. Commonly used models include Support Vector Machines (SVM), Averaged Perceptron, and Logistic Regression. However, these feature-based machine learning approaches heavily rely on feature engineering, necessitating extensive human annotation and being limited by the performance of feature extraction tools.


\subsubsection{Neural Network Approaches}
More recent research primarily utilizes neural network models. A typical approach applies a neural network model, such as an LSTM or a pre-trained transformer-based language model, to encode temporal entity pairs and their context for classification.  Given an input sequence $X = {x_1, x_2, \dots, x_n}$ with length $n$, the encoding neural network model, $f_{enc}$, produces the encoded representation of the input sequence $X$ as:
\begin{equation}
H = f_{enc}(X) = {h_1, h_2, \dots, h_n},
\end{equation}
where $H$ denotes the set of encoded hidden states, and $h_i$ represents the encoding of the $i^{th}$ token in the input sequence.

Two prevalent methods exist for obtaining temporal pair representations from the encoded context. The first method employs special tokens (e.g., [CLS] in BERT) to represent the entire input sequence and special symbols to indicate the positions of the temporal entities, as in "\textit{Cuban authorities <e>estimated</e> that 100,000 women <e>participated</e> in the march.}" The overall representation of this input sequence, $h_{CLS}$, is input to the classification layer, treating the task as a sequence classification problem.

Alternatively, temporal entity representations can be extracted from the encoded input sequence using methods such as selecting the first token of each temporal entity or employing an average pooling method. In this approach, the representations of the two temporal entities, $h_{e1}$ and $h_{e2}$, are obtained as:

\begin{align}
h_{e1} &= g_{e1}(H), \\
h_{e2} &= g_{e2}(H),
\end{align}

where $g_{e1}(H)$ and $g_{e2}(H)$ are functions extracting the representations of the first and second temporal entities, respectively, from the set of encoded hidden states $H$. 

The encoded temporal entity representations are then input to a softmax activation-based classification layer to compute probabilities for each relation. For the first method using $h_{CLS}$, the probability is computed as $p(y_i) = f_{softmax}(h_{CLS})$. For the second method using $h_{e1}$ and $h_{e2}$, the probability is computed as $p(y_i) = f_{softmax}(h_{e1}, h_{e2})$. In both cases, $p(y_i)$ represents the probability of the $i^{th}$ relation and the softmax function computes the probabilities for all relations.

Numerous approaches have been proposed to improve the neural network-based temporal classifiers, which can be categorized as integrating external knowledge and improving model robustness.

\paragraph{Incorporating Extra Knowledge}

The extra knowledge includes temporal common sense knowledge, knowledge of the label distribution of the training dataset, and knowledge acquired through external information extraction (IE) tools.

\textbf{Temporal commonsense knowledge} refers to the universal cognition of the temporal properties of things or the relations between events. It includes the information duration of events, the order of occurrence, the frequency of occurrence, and typical times of occurrence, etc. For example, the activity of "eating" usually takes place at specific times of the day and lasts for a relatively short time, while the activity of "vacationing" can last from several days to several weeks. This temporal commonsense helps us reason about the temporal relationships between events. In the task of temporal relation extraction, existing works mainly integrate temporal common sense knowledge into neural network models in two ways: first, pretraining a Siamese network on a temporal commonsense knowledge graph (such as TEMPROB and ConceptNet), and then using this network to encode the input temporal entities to enhance the representation of the pairwise temporal classifier; second, using a  neural network encoder pre-trained on the temporal knowledge graph to encode pairs of temporal entities, thus implicitly incorporating common sense information into the representation of the temporal entity pairs.

\textbf{Prior knowledge of the label distribution of the training dataset} reflects the distribution of different temporal relations. It is assumed that the distribution of temporal relationships observed during the testing phase should be similar to the distribution in the training set. In order to make the model comply with this assumption, X uses the Dirichlet prior distribution to model the distribution of temporal relationships in the training set and integrates this prior information into the training process through KL divergence loss.

\textbf{Knowledge acquired through external IE tools} refers to the structured knowledge we extract from the context of pairs of temporal entities using already trained IE models or some simple IE heuristic methods. This extracted structured knowledge is integrated into the pairwise classifier to help more accurately predict temporal relationships. Current work focuses on extracting semantic and syntactic structure information from the context, as well as document structure information, and using a graph neural network (GNN) to integrate this structural information into the pairwise classifier. For example, X uses the output of a syntactic parser and a semantic role labeler to capture dependency relationships and semantic role relations. These relations help reveal syntactic and semantic interactions between temporal entities, thus building a richer context for the representation of temporal entities. In addition, X extracts information about whether entities are in the same sentence, whether sentences are adjacent, and the subordination relationships between documents and sentences from the structure of documents and sentences. This structural information provides additional context for the model, helping to understand the relative positions and relationships of temporal entities in the text. Y uses a rhetorical structure parser to extract the rhetorical structure of the document, as well as the relations between the temporal entities and the document creation time. 

\paragraph{Enhancing Model Robustness}
Different approaches have been proposed in past work to improve the robustness of the model. These methods include Multi-tasking, Pre-training, Self-learning, Data Augmentation, ensemble-based fine-tuning, and adversarial training. In the Multi-tasking approach, apart from predicting the temporal relations between input time entities, work A also performs event extraction, work B performs event relative time prediction, work C performs general relation extraction, and work D performs event extraction, event duration, and relative time prediction. In the pre-training approach, work E collected additional pre-training data and performed mask event and temporal cue prediction as pre-training, while work F continued pre-training the BERT model on the clinical domain. In self-training, works G and H used Monte Carlo Dropout and Bayesian Active Learning by Disagreement (BALD), respectively, to select pseudo-labeled samples. In data augmentation, work I used templates to generate additional samples and performed contrastive learning, work J used distant supervision to collect additional training data, and work K generated counterfactual samples to help the model achieve better predictions. Works L and M used adversarial perturbation and ensemble-based methods, respectively, to fine-tune transformer-based models to enhance model robustness.

\subsubsection{Temporal Constraints}

% The box embedding method has a problem. It has very low performance and they compared with wrong numbers in their paper.
\begin{table}
    \centering
    \small
    \setlength{\tabcolsep}{0.5em}
    \begin{tabular}{c c}
    \toprule
    Model & F1 \\
    \midrule
    Bayesian-Trans \cite{tan2023event} & 82.7 \\
    Box Embedding \cite{hwang-etal-2022-event} & 71.1 \\
    Relative Event Time \cite{wen-ji-2021-utilizing} & 81.7 \\
    HGRU + Knowledge \cite{tan-etal-2021-extracting} & 80.5 \\
    Poincaré Event Embeddings \cite{tan-etal-2021-extracting} & 78.9 \\
    Joint Constrained Learning \cite{wang-etal-2020-joint} & 78.8 \\
    LSTM + Knowledge \cite{ning-etal-2019-improved} & 76.3 \\
    CogCompTime \cite{ning-etal-2018-cogcomptime} & 66.6 \\
    \bottomrule
    \end{tabular}
    \caption{Models' performance on MATRES dataset.}
    \label{table:err-vs-fid}
\end{table}


% Note: I need to check the dataset. Some of the previous works use different versions of TBD, but they are compared to each other.
% We should add base model to the table
\begin{table*}
    \centering
    \small
    \setlength{\tabcolsep}{0.5em}
    \begin{tabular}{c c c c}
    \toprule
    Model & E-E F1 & E-T F1 & E-DCT F1 \\
    \midrule
    Bayesian-Trans \cite{tan2023event} & 65.0/- 7 - & - \\
    DTRE \cite{wang-etal-2022-dct} & 72.3/70.2 & 70.6/67.5 & 70.6/67.5 \\
    TIMERS \cite{mathur-etal-2021-timers} &  67.8/- & - & - \\
    ECONET \cite{han-etal-2021-econet} & 66.8/- & - & - \\
    Rand \cite{cheng-etal-2020-dynamically} &  63.0/61.4 & 60.2/54.8 & 75.9/65.2 \\
    SEC \cite{cheng-etal-2020-dynamically} & -/65.0 & -/55.8 & -/65.9 \\
    GCL \cite{meng-rumshisky-2018-context} & -/57.0 & -/48.7 & -/48.9 \\
    DP-RNN \cite{cheng-miyao-2017-classifying} & -/52.9 & -/47.1 & -/54.6 \\
    BERT-base \cite{wang-etal-2022-dct} & 62.2/59.7 & 49.4/49.0 & 73.8/69.4 \\
    RoBERTa-base \cite{wang-etal-2022-dct} & 62.4/59.8 & 51.5/49.8 & 76.3/72.1 \\
    \bottomrule
    \end{tabular}
    \caption{Models’ performance on TimeBank-Dense. The figures before and after “/” refer to the results on five and six types (with/without vague). (I adapted this table from \citet{wang-etal-2022-dct}.) }
    \label{table:err-vs-fid}
\end{table*}

% \subsection{Temporal Relation Extraction}
% The goal of the temporal relation extraction is to construct a directed acyclic graph for a given text document.
% The nodes are temporal entities, which can be an event or a time.
% The edges are temporal relations.
% Most of the temporal relations used in existing works are derived from the 13 relations in Allen's interval algebra.
% Temporal relations can be grouped according to the types of temporal entities involved: 1) event-event relations, 2) event-time relations, and 3) time-time relations.
% The relations in the temporal graph need to follow two temporal-specific rules:
% \begin{enumerate}
%     \item Symmetry: Some temporal relations exhibit symmetry, such as before, after, and equal. For example, if A is before B, then B is after A. If A is equal to B, then B is also equal to A.
%     \item Transitivity: If A is before B, and B is before C, then A is before C.
% \end{enumerate}

% The typical temporal relation extraction method treats this task as a pairwise classification problem. Given two temporal entities, a classifier learns to identify the temporal relationship between them (Section x.x). Based on the pairwise classifier, existing works have proposed various methods to impose temporal rules during training and testing, aiming to improve the global consistency of the model's predictions (Section x.x). Additionally, there are a few studies that present alternative frameworks for the temporal relation extraction task, which are discussed in Section x.x.

% \subsubsection{Datasets}

% \subsubsection{Classification-based Methods}
% Using Transformer-based neural network models for temporal relation extraction is commonly framed as a text classification task involving pairs of instances.  It begins with all-time expressions and events in the text being pre-organized into pairwise relations, along with their contextual details. These paired instances and their context serve as the input to the model, with the model outputting the temporal relation between them, such as "before," "after," etc.  Specifically, given an input sequence $X = {x_1, x_2, \dots, x_n}$ with length $n$, the encoding Transformer model, $M_{enc}$, produces the encoded representation of the input sequence $X$ as:
% \begin{equation}
% H = f_{enc}(X) = {h_1, h_2, \dots, h_n},
% \end{equation}
% where $H$ denotes the set of encoded hidden states, and $h_i$ represents the encoding of the $i^{th}$ token in the input sequence.

% Two prevalent methods exist for obtaining temporal pair representations from the encoded context. The first method employs special tokens (e.g., [CLS] in BERT) to represent the entire input sequence and special symbols to indicate the positions of the temporal entities, as in "\textit{Cuban authorities <e>estimated</e> that 100,000 women <e>participated</e> in the march.}" The overall representation of this input sequence, $h_{CLS}$, is input to the classification layer, treating the task as a sequence classification problem.

% Alternatively, temporal entity representations can be extracted from the encoded input sequence using methods such as selecting the first token of each temporal entity or employing an average pooling method. In this approach, the representations of the two temporal entities, $h_{e1}$ and $h_{e2}$, are obtained as:

% \begin{align}
% h_{e1} &= g_{e1}(H), \\
% h_{e2} &= g_{e2}(H),
% \end{align}

% where $g_{e1}(H)$ and $g_{e2}(H)$ are functions extracting the representations of the first and second temporal entities, respectively, from the set of encoded hidden states $H$. 

% The encoded temporal entity representations are then input to a softmax activation-based classification layer to compute probabilities for each relation. For the first method using $h_{CLS}$, the probability is computed as $p(y_i) = f_{softmax}(h_{CLS})$. For the second method using $h_{e1}$ and $h_{e2}$, the probability is computed as $p(y_i) = f_{softmax}(h_{e1}, h_{e2})$. In both cases, $p(y_i)$ represents the probability of the $i^{th}$ relation and the softmax function computes the probabilities for all relations.

% Numerous approaches have been proposed to improve the neural network-based temporal classifiers, which can be categorized as integrating external knowledge and improving model robustness.


% \paragraph{Incorporating Extra Knowledge} The extra knowledge includes temporal common sense knowledge, knowledge of the label distribution of the training dataset, and knowledge acquired through external information extraction (IE) tools.

% \textbf{Temporal commonsense knowledge} refers to the universal cognition of the temporal properties of things or the relations between events. It includes the information duration of events, the order of occurrence, the frequency of occurrence, and typical times of occurrence, etc. For example, the activity of "eating" usually takes place at specific times of the day and lasts for a relatively short time, while the activity of "vacationing" can last from several days to several weeks. This temporal commonsense helps us reason about the temporal relations between events. In the task of temporal relation extraction, existing works mainly integrate temporal common sense knowledge into neural network models in two ways: first, pretraining a Siamese network on a temporal commonsense knowledge graph (such as TEMPROB and ConceptNet), and then using this network to encode the input temporal entities to enhance the representation of the pairwise temporal classifier; second, using a  neural network encoder pre-trained on the temporal knowledge graph to encode pairs of temporal entities, thus implicitly incorporating common sense information into the representation of the temporal entity pairs.

% \textbf{Prior knowledge of the label distribution of the training dataset} reflects the distribution of different temporal relations. It is assumed that the distribution of temporal relations observed during the testing phase should be similar to the distribution in the training set. In order to make the model comply with this assumption, X uses the Dirichlet prior distribution to model the distribution of temporal relations in the training set and integrates this prior information into the training process through KL divergence loss.

% \textbf{Knowledge acquired through external IE tools} refers to the structured knowledge we extract from the context of pairs of temporal entities using already trained IE models or some simple IE heuristic methods. This extracted structured knowledge is integrated into the pairwise classifier to help more accurately predict temporal relations. Current work focuses on extracting semantic and syntactic structure information from the context, as well as document structure information, and using a graph neural network (GNN) to integrate this structural information into the pairwise classifier. For example, X uses the output of a syntactic parser and a semantic role labeler to capture dependency relations and semantic role relations. These relations help reveal syntactic and semantic interactions between temporal entities, thus building a richer context for the representation of temporal entities. In addition, X extracts information about whether entities are in the same sentence, whether sentences are adjacent, and the subordination relations between documents and sentences from the structure of documents and sentences. This structural information provides additional context for the model, helping to understand the relative positions and relations of temporal entities in the text. Y uses a rhetorical structure parser to extract the rhetorical structure of the document, as well as the relations between the temporal entities and the document creation time. 

% \paragraph{Enhancing Model Robustness}
% Different approaches have been proposed in past work to improve the robustness of the model. These methods include Multi-tasking, Pre-training, Self-learning, Data Augmentation, ensemble-based fine-tuning, and adversarial training. In the Multi-tasking approach, apart from predicting the temporal relations between input time entities, work A also performs event extraction, work B performs event relative time prediction, work C performs general relation extraction, and work D performs event extraction, event duration, and relative time prediction. In the pre-training approach, work E collected additional pre-training data and performed mask event and temporal cue prediction as pre-training, while work F continued pre-training the BERT model on the clinical domain. In self-training, works G and H used Monte Carlo Dropout and Bayesian Active Learning by Disagreement (BALD), respectively, to select pseudo-labeled samples. In data augmentation, work I used templates to generate additional samples and performed contrastive learning, work J used distant supervision to collect additional training data, and work K generated counterfactual samples to help the model achieve better predictions. Works L and M used adversarial perturbation and ensemble-based methods, respectively, to fine-tune transformer-based models to enhance model robustness.

% \paragraph{Temporal Constraints}

% \subsubsection{Findings and Discussion}


% % The box embedding method has a problem. It has very low performance and they compared with wrong numbers in their paper.
% \begin{table}
%     \centering
%     \small
%     \setlength{\tabcolsep}{0.5em}
%     \begin{tabular}{c c}
%     \toprule
%     Model & F1 \\
%     \midrule
%     Bayesian-Trans \cite{tan2023event} & 82.7 \\
%     Box Embedding \cite{hwang-etal-2022-event} & 71.1 \\
%     Relative Event Time \cite{wen-ji-2021-utilizing} & 81.7 \\
%     HGRU + Knowledge \cite{tan-etal-2021-extracting} & 80.5 \\
%     Poincaré Event Embeddings \cite{tan-etal-2021-extracting} & 78.9 \\
%     Joint Constrained Learning \cite{wang-etal-2020-joint} & 78.8 \\
%     LSTM + Knowledge \cite{ning-etal-2019-improved} & 76.3 \\
%     CogCompTime \cite{ning-etal-2018-cogcomptime} & 66.6 \\
%     \bottomrule
%     \end{tabular}
%     \caption{Models' performance on MATRES dataset.}
%     \label{table:err-vs-fid}
% \end{table}


% % Note: I need to check the dataset. Some of the previous works use different versions of TBD, but they are compared to each other.
% % We should add base model to the table
% \begin{table*}
%     \centering
%     \small
%     \setlength{\tabcolsep}{0.5em}
%     \begin{tabular}{c c c c}
%     \toprule
%     Model & E-E F1 & E-T F1 & E-DCT F1 \\
%     \midrule
%     Bayesian-Trans \cite{tan2023event} & 65.0/- 7 - & - \\
%     DTRE \cite{wang-etal-2022-dct} & 72.3/70.2 & 70.6/67.5 & 70.6/67.5 \\
%     TIMERS \cite{mathur-etal-2021-timers} &  67.8/- & - & - \\
%     ECONET \cite{han-etal-2021-econet} & 66.8/- & - & - \\
%     Rand \cite{cheng-etal-2020-dynamically} &  63.0/61.4 & 60.2/54.8 & 75.9/65.2 \\
%     SEC \cite{cheng-etal-2020-dynamically} & -/65.0 & -/55.8 & -/65.9 \\
%     GCL \cite{meng-rumshisky-2018-context} & -/57.0 & -/48.7 & -/48.9 \\
%     DP-RNN \cite{cheng-miyao-2017-classifying} & -/52.9 & -/47.1 & -/54.6 \\
%     BERT-base \cite{wang-etal-2022-dct} & 62.2/59.7 & 49.4/49.0 & 73.8/69.4 \\
%     RoBERTa-base \cite{wang-etal-2022-dct} & 62.4/59.8 & 51.5/49.8 & 76.3/72.1 \\
%     \bottomrule
%     \end{tabular}
%     \caption{Models’ performance on TimeBank-Dense. The figures before and after “/” refer to the results on five and six types (with/without vague). (I adapted this table from \citet{wang-etal-2022-dct}.) }
%     \label{table:err-vs-fid}
% \end{table*}

% \section{Application of Temporal Information Extraction Systems}


% \section{Experiments}
% \subsection{Research Questions}

% \begin{enumerate}
%     \item Has the recently emerged closed-source large language model solved temporal relation extraction?
%     \item If we want to use an open-source large language model to solve the task of temporal relation extraction, which model should we start with, and which dataset should we use? %, not a science question
%     \item What are the main errors made by these open-source large language models (do we still need constraints)?
%     \item Have they solved in the fine-tuning setting?
%     \item Have they solved in the few-shot setting?
%     \item Which of the prior works still provide benefits in LLM (adv loss, pick the easiest method to implement)?
% \end{enumerate}

==> sections_old/time-norm.tex <==
\section{Time Expression Extraction and Normalization}
